Constraints on Dark Matter Self-Interactions from weak lensing of galaxies from the Dark Energy Survey around clusters from the Atacama Cosmology Telescope Survey

Self--interactions of dark matter particles impact the distribution of dark matter in halos. The exact nature of the self--interactions can lead to either expansion or collapse of the core within the halo lifetime, leaving distinctive signatures in the dark matter distributions not only at the halo center but throughout the virial region. Optical galaxy surveys, which precisely measure the weak lensing of background galaxies by massive foreground clusters, allow us to directly measure the matter distribution within clusters and probe subtle effects of self--interacting dark matter (SIDM) throughout the halo's full radial range. We compare the weak--lensing measurements reported by Shin et al. 2021, which use lens clusters identified by the Atacama Cosmology Telescope Survey and source galaxies from the Dark Energy Survey, with predictions from SIDM models having either elastic or dissipative self--interactions. To model the weak--lensing observables, we use cosmological N-body simulations for elastic self--interactions and semi-analytical fluid simulations for dissipative self--interactions. We find that current weak--lensing measurements already constrain the isotropic and elastic SIDM to a cross-section per mass of $\sigma/m<1~{\rm cm^2/g}$ at a $95\%$ confidence level. The same measurements also impose novel constraints on the energy loss per unit mass for dissipative SIDM. Upcoming surveys are anticipated to enhance the signal-to-noise of weak--lensing observables significantly making them effective tools for investigating the nature of dark matter, including self--interactions, through weak lensing.

==> hyperlink-year-only-natbib-patch.tex <==
% found on https://tex.stackexchange.com/questions/23227/how-to-hyperlink-only-the-year-part-when-using-natbib-and-hyperref

\RequirePackage{hyperref}
\RequirePackage{natbib}
\RequirePackage{etoolbox}

\makeatletter

% Patch case where name and year are separated by aysep
\patchcmd{\NAT@citex}
  {\@citea\NAT@hyper@{%
     \NAT@nmfmt{\NAT@nm}%
     \hyper@natlinkbreak{\NAT@aysep\NAT@spacechar}{\@citeb\@extra@b@citeb}%
     \NAT@date}}
  {\@citea\NAT@nmfmt{\NAT@nm}%
   \NAT@aysep\NAT@spacechar\NAT@hyper@{\NAT@date}}{}{}

% Patch case where name and year are separated by opening bracket
\patchcmd{\NAT@citex}
  {\@citea\NAT@hyper@{%
     \NAT@nmfmt{\NAT@nm}%
     \hyper@natlinkbreak{\NAT@spacechar\NAT@@open\if*#1*\else#1\NAT@spacechar\fi}%
       {\@citeb\@extra@b@citeb}%
     \NAT@date}}
  {\@citea\NAT@nmfmt{\NAT@nm}%
   \NAT@spacechar\NAT@@open\if*#1*\else#1\NAT@spacechar\fi\NAT@hyper@{\NAT@date}}
  {}{}

\makeatother

